Evaluation of CNN-based Automatic Music Tagging Models

Recent advances in deep learning accelerated the development of content-based automatic music tagging systems. Music information retrieval (MIR) researchers proposed various architecture designs, mainly based on convolutional neural networks (CNNs), that achieve state-of-the-art results in this multi-label binary classification task. However, due to the differences in experimental setups followed by researchers, such as using different dataset splits and software versions for evaluation, it is difficult to compare the proposed architectures directly with each other. To facilitate further research, in this paper we conduct a consistent evaluation of different music tagging models on three datasets (MagnaTagATune, Million Song Dataset, and MTG-Jamendo) and provide reference results using common evaluation metrics (ROC-AUC and PR-AUC). Furthermore, all the models are evaluated with perturbed inputs to investigate the generalization capabilities concerning time stretch, pitch shift, dynamic range compression, and addition of white noise. For reproducibility, we provide the PyTorch implementations with the pre-trained models.

==> sss_Dataset.tex <==
\section{Dataset}\label{sec:dataset}
\subsection{MagnaTagATune}

MagnaTagATune (MTAT) is one of the most broadly used datasets for benchmarking automatic music tagging systems. It contains multi-label annotations of genre, mood and instrumentation for 25,877 audio 30 seconds long segments. The audio is in MP3 format (32 Kbps bitrate and 16 KHz sample rate). Originally the dataset is split into 16 folders, and commonly the first 12 folders are used for training, the 13th for validation and the last three are used for testing. Only 50 most frequent tags are typically used for the task. The top 50 tags include genre and instrumentation labels, as well as decades (e.g., '80s' and '90s') and moods.

In our work, we follow the same data split and we use the top 50 tags to be consistent with results reported in the majority of previous studies \footnote{\url{https://github.com/jongpillee/music_dataset_split/tree/master/MTAT_split}}. However, we have noted that the performances reported in some of the studies are inconsistent, as some authors discarded segments without any associated tags and others do not. This lead to slightly higher values of performance. Some previous works re-using those reports are unintentionally comparing incompatible performance values which is one of the main motivations of this work.

\subsection{Million Song Dataset}

The MSD~\cite{bertin2011million} is a dataset that originaly only contained audio features, it was later expanded by the MIR community with information including tags, lyrics and other annotations. 
This dataset also contains a subset mapped to 30 seconds audio previews available at the service 7digital\footnote{\url{https://www.7digital.com}} wich not possible to access anymore. For this subset of songs the MSD has collaborative tags that are originally from Lastfm.\footnote{\url{https://www.last.fm}} In total the subset contains 241,904 annotated track fragments, which is commonly used for benchmark for music auto-tagging systems. These tags cover genre, instrumentation, moods and eras. The audio fragments vary in quality, they are encoded as MP3 with and the bitrate rages from 64 to 128 Kbps, the sample rates is 22 KHz or 44 KHz. 

Again, in our study we follow the dataset split commonly used by researchers\footnote{\url{https://github.com/jongpillee/music_dataset_split}}~\cite{lee2017sample,pons2018end} and use only 50 most frequent tags for consistency with previous studies. This split includes 201{,}680 tracks for training, 11{,}774 for validation and 28{,}435 for testing. Unfortunately, similarly to MTAT, some previous studies report inconsistent comparisons of auto-tagging approaches, as there also exists another slightly different split,\footnote{\url{https://github.com/keunwoochoi/MSD_split_for_tagging}} containing audio files smaller than 29s and lowering performance values. 

One of the challenges in music tagging is because of copyright issues is difficult to have a large collection of annotated audio. The annotations for the MSD that are commonly use for this task are originally from last.fm, since they are crowdsourced, they are very noisy. 
For example, one of the problems is that the songs are weakly labeled \cite{choi2017effects}, i.e: the absence of a tag in a song does not mean that the song should not have the tag.


\subsection{MTG-Jamendo Dataset}

The MTG-Jamendo Dataset contain audio of 55,701 full music tracks. The minimum duration of each track is 30 seconds, in MP· format with 320kbps bitrate. From this we see that this dataset contains larger samples of audio, with higher quality. The dataset contains annotations for all the tracks with 692 different tags, but also the annotations for the top 50 tags are provided. 

The authors of the dataset provide multiple splits of the data for training, validation and test. In this work we use the split with \hl{TODO} only for the top 50 tags. The motivation to use this dataset is that was recently released so there are not many publications that reporting the performance of the architectures in this dataset. Also, there are different characteristics in MTG-Jamendo Dataset comapred  with the MSD and MagnaTagATune, which could lead to different performance of the architectures.


